CurveCloudNet: Processing Point Clouds with 1D Structure

Modern depth sensors such as LiDAR operate by sweeping laser-beams across the scene, resulting in a point cloud with notable 1D curve-like structures. In this work, we introduce a new point cloud processing scheme and backbone, called CurveCloudNet, which takes advantage of the curve-like structure inherent to these sensors. While existing backbones discard the rich 1D traversal patterns and rely on generic 3D operations, CurveCloudNet parameterizes the point cloud as a collection of polylines (dubbed a "curve cloud"), establishing a local surface-aware ordering on the points. By reasoning along curves, CurveCloudNet captures lightweight curve-aware priors to efficiently and accurately reason in several diverse 3D environments. We evaluate CurveCloudNet on multiple synthetic and real datasets that exhibit distinct 3D size and structure. We demonstrate that CurveCloudNet outperforms both point-based and sparse-voxel backbones in various segmentation settings, notably scaling to large scenes better than point-based alternatives while exhibiting improved single-object performance over sparse-voxel alternatives. In all, CurveCloudNet is an efficient and accurate backbone that can handle a larger variety of 3D environments than past works.

==> content/main/figures/teaser.tex <==
\begin{figure*}[t]
    % \centering
    \includegraphics[width=1.0\textwidth]{content/main/images/banner.jpg}
    \caption{Visualizations of CurveCloudNet's segmentation prediction (left) and the input curve cloud (right) for each of our five evaluation datasets. Each dataset exhibits distinct size, structure, and laser scanning pattern, as communicated in \cref{tab:summary-results-and-datasets} \todo{How do we put this at the top of the paper??!}
    }
    \label{fig:teaser}
    \vspace{-2mm}
\end{figure*}

==> content/main/tables/summer-robotics.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{4pt}
\centering
\scalebox{0.82}{
    \begin{tabular}{ l c | c | c c c c c c c | c c c }
    \toprule
    & &  \textbf{{ShapeNet}} & \multicolumn{7}{c}{\textbf{{\kortx Dataset}} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{{\kortx Performance}} ($\downarrow$)} \\
    \textbf{Method} & Type & mIOU ($\uparrow$) & mIOU & Cap & Chair & Earphone & Knife & Mug & Rocket & Time \scriptsize (ms) & GPU \scriptsize (GB) & Param \scriptsize (M) \\
    \midrule
    % PointNet~\cite{Qi2017CVPR} & 63.1 \scriptsize $\pm$ 0.4 & 68.5 \scriptsize $\pm$ 1.8 & 77.1 & 80.1 & 62.5 & 62.9 & 56.0 & 72.4 & \textbf{10} & \textbf{0.29} & 1.49 \\
    PointNet++~\cite{Qi2017NIPS} & Point & 66.9 \scriptsize $\pm$ 1.2 & 71.0 \scriptsize $\pm$ 2.5 & 69.3 & 65.9 & 83.1 & 70.4 & 71.7 & 65.5 & 109 & 1.95 & 1.53\\
    DGCNN~\cite{Wang2019SIGGRAPHb} & & 64.6 \scriptsize $\pm$ 0.8 & 73.3 \scriptsize $\pm$ 0.9 & 73.0 & 76.6 & 81.1 & 79.6 & 58.3 & 71.2 & 143 & 1.45 & 2.18 \\
    CurveNet~\cite{Xiang2021ICCV} & & 68.4 \scriptsize $\pm$ 0.7 & 71.5 \scriptsize $\pm$ 0.4 & 80.9 & \textbf{89.7} & 63.6 & 63.0 & 68.0 & 64.0 & 227 & 1.16 & 5.33 \\
    PointMLP~\cite{Ma2022ICLR} & & 72.1 \scriptsize $\pm$ 0.4 & 75.4 \scriptsize $\pm$ 1.3 & 77.2 & 75.3 & 78.8 & 83.1 & 64.6 & 73.6 & 58 & 0.83 & 16.76 \\
    PointNext~\cite{Qian2022PointNeXtRP} & & 69.8 \scriptsize $\pm$ 0.6 & 73.7 \scriptsize $\pm$ 0.5 & \textbf{82.2} & 75.9 & 80.9 & 68.3 & 70.8 & 63.9 & 81 & 1.69 & 13.8 \\
    \hline
    % PVCNN~\cite{Liu2019NeurIPS} ~ & 71.2 \scriptsize $\pm$ 0.9 & 77.6 \scriptsize $\pm$ 1.4 & \textbf{82.0} & 79.9 & 71.7 & 72.4 & \textbf{83.3} & \textbf{74.4} & 36 & 1.85 & 4.20\\
    MinkowskiNet~\cite{Choy2019CVPR} & Voxel & 62.9  \scriptsize $\pm$ 1.7 & 60.1 \scriptsize $\pm$ 1.4 & 67.5 & 53.2 & 74.3 & 56.4 & 73.6 & 27.5 & 42 & 0.21 & 36.62 \\ 
    Cylinder3D~\cite{Zhou2020ARXIV} & & 58.6 \scriptsize $\pm$ 0.5 & 63.5  \scriptsize $\pm$ 0.2 & 64.8 & 56.9 & 80.8 & 55.1 & 64.8 & 58.7 & 96 & 5.76 & 56.03 \\
    SphereFormer~\cite{lai2023spherical} & &  67.6 \scriptsize $\pm$ 0.9 & 69.7 \scriptsize $\pm$ 1.3 & 71.5 & 65.1 & 86.0 & 59.6 & 67.2 & \textbf{79.5} & 38 & 0.25 & 32.3\\
    \hline
    % Cylinder3D (Ours) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --\\\hline
    CurveCloudNet & Curve & \textbf{73.0 \scriptsize $\pm$ 0.9} & \textbf{78.9 \scriptsize $\pm$ 1.1} & 69.1 & 87.3 & \textbf{86.7} & \textbf{87.0} & \textbf{74.7} & 67.8 & 77 & 1.01 & 8.74\\

    \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \caption{\textit{Object Segmentation Results.} Class-average mIOU is reported for synthetic ShapeNet and real-world \kortx data. CurveCloudNet achieves the highest accuracy compared to point and voxel baselines. Performance is on an Nvidia RTX 3090 GPU (batch size 16).}
    \label{tab:summer-robotics}
\end{table*}

==> content/main/tables/teaser-dataset-table.tex <==
\begin{table}
\centering
\scalebox{0.84}{
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ l | c c c c | c }
\toprule
& ShapeNet & KortX & A2D2 & nuScenes & Average \\
  \midrule
  \multicolumn{1}{l}{\textit{Dataset Statistic}} & & & \\
  location & Synthetic & Indoor & Outdoor & Outdoor \\
  scale & $\pm$ 1 & $\pm$ 2m & $+$ 70m  & $\pm$ 50m\\
  laser pattern & ALL & Random & Grid & Parallel \\
  \# points & 2048 & 2048 & $\sim$ 5K & $\sim$ 15K \\
  % \# classes & 50 & 15 & 13 & 17 \\
  \# train & 12K & 6K & 18K & 28K\\
\midrule
%
  \multicolumn{1}{l}{\textit{Model mIOU}} & & & \\
  % CurveNet~\cite{Xiang2021ICCV} & 71.5 & 79.6 & 4.4 & -- & 51.8 \\
  PointMLP~\cite{Ma2022ICLR} & 75.4 & 79.3 & 47.6 & 67.9 & 67.6  \\ 
  PointNext~\cite{Qian2022PointNeXtRP} & 73.7 & 79.9 & 38.6 & 55.7 & 62.0\\
  Cylinder3D~\cite{Zhou2020ARXIV} & 63.5 & 77.6 & 53.0 & 76.1 & 67.6\\
  SphereFormer~\cite{Sphereformer} & \todo{XX}\\ \hline
  CurveCloudNet & 73.0 & 81.9 & 53.6 & 77.3 & \textbf{71.5}\\
\end{tabular}}
\vspace{1mm}
\caption{\textit{Dataset Comparison.} }
\label{tab:a2d2-ablation}
\vspace{-3mm}
\end{table}

==> content/main/text/02_intro.tex <==

\section{Introduction}
\label{sec:intro}
\input{content/main/figures/teaser}

% modern sensors exhibit curve patterns but not being utilized
% We introduce a novel point cloud processing scheme designed to exploit the curve-like structures of the 3D sensors. The resulting point cloud processing backbone, dubbed Curbenet is efficient, scalable, and expressive in terms of accuracy. 
% At the core of CruveCloudNet lies 

% 3D sensors useful in many applications
% Effectively processing the output of 3D sensors is essential for 3D-aware scene understanding with important applications in autonomous driving and robotics.
%       many sensors output point clouds with special structure from scanning, curves. (e.g in fig...)
Many modern 3D sensors such as \lidar operate by sweeping laser-beams across the scene. As the laser traverses object surfaces, it returns dense measurements along the scanning direction, resulting in a 3D point cloud with notable curve-like structures (see \cref{fig:overview}). 
While the computer vision community has proposed various backbones for processing 3D point clouds for fundamental tasks such as semantic segmentation \cite{Qi2017CVPR, Qi2017NIPS, Wang2019SIGGRAPHb, Thomas2019ICCV, Hu2020CVPR}
and object detection \cite{Wu2022GeosciRemoteSens, Wang2021NeurIPS, Wu2022ARXIV, Wu2022CVPR, Yang2022ECCV}, 
they rarely make use of the innate curve-like structures of the scanner outputs. 


%
%
% along the curves utilizing the fixed spatial order of curve points. %Additionally, our backbone can account for arbitrary 1D geometric structure, a capability that is increasingly important as laser-scanners such as LiDAR become more dynamic and controllable in their scanning. %, \colton{not sure if the following part makes sense}, \ie it enables the best of both worlds from object-level and scene-level reasoning.efficient, scalable, and highly accurate, achieving advanced segmentation results on both objects and large scenes

Concretely, existing 3D backbones can be generally characterized as point-based, which operate directly on the scanned point cloud, or discritization-based, which discretize 3D space into voxels or 2D projections.
Backbones that directly operate on 3D points \cite{Qi2017NIPS, Su2018CVPR, Hua2018CVPR, Wang2018CVPRb, Xu2018ECCV, Esteves2018ECCV,
Wu2019CVPR, Thomas2019ICCV} typically exchange and aggregate point features in Euclidean space, and have shown success on several downstream tasks (\eg semantic segmentation, shape classification, \etc) for individual objects or relatively small indoor scenes. These methods, however, do not scale well to large scenes (\eg in outdoor settings) due to inefficiencies in processing large unstructured point sets. On the other hand, recent descritization approaches such as sparse voxel-based methods \cite{Wu2018ICRA, Su2018CVPR, Graham2018CVPR, Choy2019CVPR,
Liu2019NeurIPS, Zhou2020ARXIV, Hu2020CVPR, Zhang2022ARXIV} rely on efficient sparse data structures that scale better to large scenes. However, they require additional memory and, for small point sets, often incur discretization error and latency overhead.

% While for the past decade this trend was fine, 
In the past, using a distinct 3D architecture for different settings was sufficient because the applications on 3D vision were more contrained - autonomous vehicles do not leave roads, manufacturing robots do not leave warehouses, and quality-assurance systems do not reason past a tabletop. However, as we push into more dynamic settings in areas such as open-world robotics, it becomes essential to build a 3D archicture that can be trained off-the-shelf for any environment.


In this work, we present a novel point cloud processing scheme designed to explicitly consider the curve-like structure of 3D sensor outputs. Instead of treating each point independently, we parameterize the point cloud as a collection of polylines, \ie curves. As a result, we establish a local structure on the points, allowing for efficient and cache-local communication between points along a curve. Additionally, the local ordering injects a lightweight and flexible curve-aware prior into the network. We propose a new backbone, CurveCloudNet, that applies 1D operations along curves. CurveCloudNet is efficient, scalable, and accurate, and outperforms existing segmentation and classification pipelines in various settings: this including indoor, outdoor, object-centric, scene-centric, sparsely scanned, and densely scanned scenes, where each setting exhibits unique laser scanner patterns (see \todo{Supp. tab 3} for example scanning patterns).
% todo: add in open world robotics!

% Additionally, sensors with irregular and unpredictable sampling densities can lead to challenges in discretization,
%
% for certain geometries; discards informtion
%
% as previous works have noted in the case of fine structures \cite{Lei2019CVPR} or cylindrical patterns \cite{Zhou2020ARXIV}. 
%
% Furthermore, the sparse (or dense) voxel data structure incurs an unnecessary memory footprint for object or small scene . % are often specifically tailored for the circular sweeping LiDAR patterns, and therefore do not generalize well to other scene types or scanning patterns, \eg segmenting small objects.

Our proposed \arch combines 1D curve reasoning with established point-based operations to achieve the best of both points and voxels. That is, curve reasoning makes our backbone scalable, accurate, and efficient for both objects and large-scale scenes and across many scanning patterns. To the best of our knowledge, our work is the first to experimentally showcase accurate and efficient predictions on \emph{both} object-level and outdoor datasets. 
%
\todo{is this next sentence too negative?}
Intuitively, \arch echos a story of strategic specialization - by leveraging the intrinsic curve structure of laser-scanned data, we can improve perception for this common medium. 
%
% We, in contrast, can achieve this flexibility by imposing a local 1D structure on the points that is consistent with the sensor's mode of data capture. % and flexible scalability compared to previous point-based methods, while also outperforming sparse-voxel methods on both objects and outdoor datasets. 
% improve accuracy over previous point-based methods without specific LiDAR patterns assumed by voxel-based methods. 
% Notably, on scene-level LiDAR segmentation, CurveCloudNet scales significantly better than any of the previous point-based methods and even performs competitively with sparse-voxel methods while maintaining a smaller GPU memory footprint. 

The essence of 1D curve reasoning is a novel adaptation of three standard point cloud operations for 1D curve structures: (1) a \textit{symmetrical 1D convolution} that operates along curves, (2) a \textit{ball grouping} similar to PointNet++ \cite{Qi2017NIPS} that groups points along curves, and (3) an efficient \textit{1D farthest-point-sampling} algorithm on curves.
Carefully integrated together with state-of-the-art point-based operations \cite{Qian2022PointNeXtRP, Ma2022ICLR, Wang2019SIGGRAPHb, Qi2017NIPS}, CurveCloudNet is a versatile, efficient, and high-performing backbone that uses little GPU memory (see \cref{fig:teaser}).

We evaluate CurveCloudNet on both object-level and outdoor scene-level datasets. For the object part segmentation task, we use ShapeNet \cite{Chang2015ARXIV, Yi2016ToG} along with a new object-level dataset, captured with the \kortx laser \cite{summer-robotics}; the latter includes real-world data of objects scanned in a curve-like manner. For the outdoor semantic segmentation task, we use the nuScenes~\cite{Caesar2020CVPR} and Audi Autonomous Driving (A2D2)~\cite{Geyer2020ARXIV} datasets. The A2D2 dataset offers a unique sensor configuration resulting in a grid-like scanning pattern, which is distinct from previous LiDAR datasets \cite{Geiger2012CVPR, Caesar2020CVPR, Chang2019CVPR, Sun2020CVPR}. Supplementary experiments on object classification demonstrate flexibility to other perception tasks. Our evaluations demonstrate that using curve structures leads to improved performance on all experiments.

% Concretely, given the laser-scanned point cloud input, we propose converting it into a \emph{curve cloud} defined as an unordered set of 1D polylines.
% As shown in \cref{fig:teaser}, the curve cloud links together points on a surface that were captured in quick succession and close spatial proximity by the scanner.
% This 3D representation maintains the resolution of the original point cloud, and also provides more information to a network by hinting at detailed geometric properties such as surface connectivity, boundaries, curvatures, and tangents.
% Moreover, a curve cloud can be processed efficiently because there are far fewer curves than points and points along a curve have a fixed spatial ordering.

% curve operations and curve backbone
% To efficiently process a curve cloud, we adapt three common point cloud operations to run on curves: (1) \textit{ball grouping} similar to PointNet++ \cite{pointnet2} to group points along curves for processing, (2) a \textit{symmetric 1D convolution} that runs along curves, and (3) an efficient furthest-point-sampling algorithm along curves.
% We incorporate these layers into a novel backbone called CurveCloudNet, which combines curve operations with existing point-based operations \cite{dgcnn, pointnet2, pointmlp, randlanet}.

% \colton{TODO: Rework the following 2 paragraphs (or integrate them into the first 4).}
% To put the versatility of CurveCloudNet in context, existing backbones that directly process points in the Euclidean space, including PointNet-variants~\cite{pointnet,pointnet2}, KPConv~\cite{kpconv}, DGCNN~\cite{dgcnn}, and attention-based methods~\cite{pointtransformer, point4dtransformer}, are adopted mainly to segment individual objects or small indoor scenes. These methods do not scale well to large outdoor scenes (\eg, self-driving settings) due to inefficiency in processing a large number of points or low accuracy due to overly-coarse processing. 


% point-based approaches useful for object-level and small indoor scenes. Detailed. but don't leverage curves, and don't scale. Also mostly tested on nice uniform point clouds like shapenet, not so much real-world scans?
% Several point-based backbones have been proposed to process such 3D data including PointNet~\cite{pointnet,pointnet2}, convolutional~\cite{kpconv}, graph-based~\cite{dgcnn}, and attention-based~\cite{pointtransformer, point4dtransformer} methods. 
% These approaches excel at capturing the details needed to segment individual objects or small indoor scenes by operating directly on points and leveraging hierarchical structures. However, these methods are usually designed for uniformly-sampled point cloud inputs and ignore sensor-specific information. Additionally, these methods cannot scale to large outdoor scenes (\eg, self-driving settings) due to the massive number of points. 

% recently sparse voxels have dominated large outdoor scenes (like self-driving) b/c of efficiency. though some methods (cylinder3d) are tailored to a specific structure like lidar, the voxelization process inherently destroys detailed info and this doesn't generalize to other sensors. 
% For large scenes, sparse voxel-based methods~\cite{sparse-voxs} tend to significantly outperform point-based methods likely due to the use of efficient sparse data structures that effectively capture the coarse structure of large outdoor scenes. However, sparse voxel-based representations are often specifically designed for the circular sweeping nature of \lidar in many driving datasets, with some methods even adopting polar coordinates \cite{polarnet} or cylindrical convolutions \cite{cyl3d} that do not generalize well to other scene-types or scanning patterns.

% in this work, we propose to explicitly leverage the curve-like structure of laser scanners and bridge the gap between point and sparse-voxel methods. Our method works well both at object-level due to ability to capture detailed curve info, and efficiently scales to large outdoor scenes with extremely efficient curve operations. 
% In this work, we propose a 3D representation and neural network backbone that explicitly leverages the curve-like 1D structure found in laser-scanned point clouds.
% By treating the point cloud as a set of polylines, our backbone can maintain full-resolution details, scale to large scenes, and account for arbitrary 1D geometric structure, \ie getting the best of both worlds from object-level point-based approaches and scene-level sparse-voxel methods.
% For the semantic segmentation task, exploiting curve structures gives better accuracy than other point-based approaches and generalizes better than a recent sparse-voxel method with reduced VRAM usage.

% curve-cloud: summary, why we expect it to help intuitively (geometric properties)


% key findings / improvements: beat others on object-level, scales to scene-level to be competitive with voxel but generalizes better with lower GPU usage to lidar and event laser sampling patterns
% Moreover, our backbone generalizes better than \lidar-specific sparse-voxel methods to handle arbitrary scanning patterns.

% contributions
In summary, we make the following \textbf{contributions}: 
\textbf{(1)} we propose operating on laser-scanned point cloud data using a \emph{curve cloud} representation, \textbf{(2)} we adapt common point cloud operations, including the ball grouping, convolution, and farthest point sampling, to efficiently run on curve clouds, \textbf{(3)} we design a novel backbone, CurveCloudNet, that makes use of both curve and point operations, and \textbf{(4)} \textcolor{red}{update to emphasize generality across many settings} we show state-of-the-art segmentation results on real-world data captured for both objects and large-scale scenes with various scanning patterns.
% \begin{itemize}
%     \setlength\itemsep{0.1em}
%     \item We propose operating on laser-scanned point cloud data using a \emph{curve cloud} representation.
%     \item We adapt common point cloud operations, including the ball grouping, convolution, and farthest-point sampling, to efficiently run on curve clouds.
%     \item We design a novel backbone, CurveCloudNet, that makes use of both curve and point operations.
%     \item We show state-of-the-art segmentation results on real-world data captured for both objects and large-scale scenes with various scanning patterns. 
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Reasoning over and understanding the output of 3D sensors is essential for a variety of applications, including modern robotics, autonomous vehicles, topographic mapping, 3D quality control, and more. Due to its simplicity and universality, most deep-learning 3D backbones assume that sensors output a point cloud. 
% %
% Consequently, researchers have proposed a myriad of different 3D backbones for processing and understanding point cloud data.
% %
% Early on, researchers converted point clouds dense voxel grids \cite{a-lot-of-stuff}, although dense voxels were quickly regarded as computationally cumbersome. 
% %
% Beginning with PointNet \cite{pointnet}, many works turned to directly reasoning on 3D point clouds \cite{point-cloud-works}.
% %
% These point cloud backbones incorporated hierarchical reasoning \cite{pn2}, adapted convolutions to point clouds \cite{dgcnn, kpconv}, incorporated geometric priors  \cite{deltaconv, diffusionnet}, used self-attention \cite{pointtransformer, point4dtransformer}, and more \cite{others}.
% %
% In recent years, researchers adapted \textit{sparse} voxelization of 3D data for larger scene-level scans \cite{sparse-voxs}.
% %
% % In contrast to point-based methods, sparse voxel backbones are able to run expressive convolutional operations that can scale to larger scenes.

% %
% However, different 3D sensors perform 3D measurements in different ways, and as general-use 3D backbones matured, a variety of works turned to sensor-specific architectures. % and task-specific architectures.
% %
% For RGBD cameras, many works applied 2D convolutions directly on the image plane instead processing on 3D point clouds \cite{rgbd-works}. 
% % 
% Similarly, researchers had success projecting 360-degree ``sweeping" LiDAR into a 2D range view; this became and still is popular for very low-latency tasks. 
% %
% Additionally, many sparse-voxel LiDAR backbones use polar coordinates \cite{polarnet}, and cylindrical convolutions \cite{cyl3d} to better capture the circular sweeping nature of the sensor.
% %
% % In intrinsic tasks such as mesh correspondence and protein classification, recent works propose 2D surface convolutions to better understand geodesic properties \cite{mesh_cnn, diffusionnet, others}.
% %
% % Finally, a collection of research has modified backbones for 4D inputs \cite{spot-and-others}, high-frequency information  \cite{siren-and-others}, rotation-equivariance \cite{congyue}, medical imaging \cite{something}, and more.

% In this work, we follow the trend of sensor-specific architectures. 
% %
% However, unlike previous methods, we are interested in a developing a 3D backbone that can flexibly address a broad set of 1D sampling structures resulting from a variety of laser-based 3D scanners. 
% %
% Specifically, a variety of 3D sensors sweep laser-beams across surfaces. 
% %
% This is especially the case for 3D sensors that recover high-fidelity or long-range measurements, such as LiDAR, classic laser scanners, and event-based laser scanners. 
% %
% Due to the lasers' traversals, these sensors acquire dense 3D measurements \textit{in a laser's direction}; in the plane orthogonal to a laser's motion, no 3D information is captured.
% %
% This results in a rich 1D structure that is shared among all these sensors.

% We propose a 3D representation and backbone that makes use of the 1D sampling structure. 
% %
% Instead of treating each point equally, we convert the point cloud into and reason over a ``curve cloud", i.e. an unordered set of 1D polylines that encodes the sequential capturing and spatially proximity of adjacent points.
% %
% As observed in \cref{fig:teaser}, a curve cloud offers a flexible structure, greater efficiency, and greater information than the original point cloud.
% %
% We adapt three classic perception operations to run on curves.
% %
% First, we adapt the ball grouping outlined in PointNet++ \cite{pointnet2} to operate on curves.
% %
% Second, we define a symmetric 1D convolution that runs along curves.
% %
% Third, we implement an efficient furthest-point-sampling algorithm along curves.
% %
% Finally, we propose a novel backbone, CurveCloudNet, that combines the three aforementioned curve operations with existing point-based operations \cite{dgcnn, pointnet2, pointmlp, randlanet}.

% On real-world object part segmentation, CurveCloudNet improves accuracy over previous methods while maintaining low latency and GPU memory usage. 
% %
% On scene-level LiDAR segmentation, CurveCloudNet significantly outperforms previous point-based methods, lowers the GPU memory footprint compared to sparse-voxel methods, and generalizes across domains better than all methods.

% In summary, our contributions are as follows:
% %
% \begin{enumerate}
%     \item We propose the restructuring of laser-scanned point cloud data into a ``curve cloud".
%     \item We adapt common perception operations, including the ball grouping, convolution, and farthest-point-sampling, to efficiently run on curve clouds.
%     \item We design a novel backbone, CurveCloudNet, that makes use of both curve and point operations.
%     \item We show state-of-the-art the object-level segmentation on real-world data captured from the KortX sensor
%     \item We show state-of-the-art scene-level segmentation on the Audi Autonomous Driving Dataset and the nuScenes Dataset.
% \end{enumerate}


==> content/main/text/04_method.tex <==


\section{Method: Learning on Curve Clouds}
Our method takes as input a 3D point cloud, parses it into a curve cloud representation, and then processes the resulting curves for perception tasks by leveraging specialized curve operations, as shown in \cref{fig:overview}. We focus on object part segmentation, semantic scene segmentation, and object classification, although in principle, our method is suitable for any other point cloud perception task. 
% BELOW: REMOVED TO SAVE SPACE!
% We begin by describing how curve clouds are constructed and summarize their key advantages (\cref{sec:prelims}). 
% Next, we detail several new operations to effectively process curve clouds (\cref{sec:curve-ops}) and finally we introduce our novel architecture built upon these curve operations (\cref{sec:curvecloudnet}).

\input{content/main/figures/architecture.tex}

\subsection{Constructing Curve Clouds} \label{sec:prelims}
\paragraph{Problem Formulation}
The input to our model is the output of a laser-based 3D sensor represented as a point cloud $P = \{p_1, p_2, ..., p_N\}$, where $p_i = [x_i, y_i, z_i]$ refers to the 3D coordinates of the $i$-th point.
For each point, we are also given an associated acquisition timestamp $t_i$ and an integer laser beam ID $b_i \in [1, B]$, which are readily available from sensors like \lidar and are helpful in extracting curve information.
For a scanner with $B$ unique laser beams, $b_i$ indicates which beam captured the point while $t_i$ gives the ordering in which points were captured.
Timestamps differ only by microseconds and indicate point ordering for constructing the curve cloud; otherwise, the point cloud is treated as an instantaneous capture of the scene.

We assume that each laser beam in the scanner captures 3D points \textit{sequentially} and at a \textit{high sampling rate} as it sweeps the scene.
Concretely, if points $p_1$, $p_2$, and $p_3$ are recorded consecutively by beam $b$, then their timestamps are ordered $t_1{<}t_2{<}t_3$. 
Moreover, if two consecutive points are spatially farther apart than some small threshold $\delta$, we assume there is a surface discontinuity and the points lie on different surfaces in the scene.


\paragraph{Curve Clouds}
A curve $c_j = [p_1, ..., p_{N_j}]$ is defined as a sequence of $N_j$ points where consecutive point pairs are connected by a line segment, \ie, a \textit{polyline}. 
The curve is bi-directional and is equivalently defined as $c_j = [p_{N_j}, p_{N_j-1}, ..., p_1]$.
A \textit{curve cloud} $C = \{c_1, ..., c_M\}$ is an unordered set of $M$ curves where each curve may contain a different number of points.
In practice, we can store a curve cloud $C$ as an $N \times 3$ tensor of points, with an additional $ptr$ tensor of length $M$ that specifies the indices where one curve ends and the next begins.
Converting the input point cloud $P$ to a corresponding curve cloud is straightforward and extremely efficient.
Points from each beam $b_i$ are ordered by  timestamp and split into curves based on distances between consecutive points.
If the distance between two consecutive points is more than a set threshold $\delta$ while traversing the points in time order, then the current curve ends and a new curve begins, \ie, a surface discontinuity has occurred.
In practice, we parallelize this process across all points and laser beams on the GPU.
More details regarding the conversion process are provided in the supplement.

% TODO
\noindent \textbf{Why Use Curves?} \label{subsec:why-curves}
Curve clouds inherit the benefits associated with the 3D point cloud representation including lightweight data structures, low memory usage, and no need to discretize the space. 
But operating on curve clouds also has several advantages over point clouds.
Point clouds are highly unstructured, making operations like nearest neighbor queries and convolutions expensive. 
Curve clouds add structure through point ordering along the polylines, allowing curves to be treated as 1D grids that permit greater cache-locality, constant-time neighborhood queries, and efficient convolutions.
This structure is flexible to any laser scanning pattern unlike, \eg, cylindrical voxel grids and polar range-view projections. % that are only suitable for \lidar.
In principle, the curve structure should also bring out the geometric properties of the surface it represents, such as curvature, tangents, and boundaries.
% For instance, the endpoints of curves represent boundaries of the surface, while the interior traversal of curves captures surface curvature and tangents.


\subsection{Operating on Curves} \label{sec:curve-ops}
We now discuss the fundamental operations for curves.
These operations are inspired by point cloud processing counterparts, so we start by reviewing operations on points.

% We define three neural operations on 1D curves: 1D farthest point sampling, 1D groupings and feature propagation, and symmetric 1D convolutions.

\vspace{-2mm}
\subsubsection{Review of Point Cloud Layers} 
\vspace{-1mm}
\label{subsec:point-review}
Many of our curve operations are inspired by point operations introduced in PointNet++~\cite{Qi2017NIPS}.
%and DGCNN~\cite{Wang2019SIGGRAPHb}. 
In particular, PointNet++ relies on \textit{sampling}, \textit{grouping}, and \textit{feature interpolation}.
We briefly review these relevant operations. % and refer the reader to the original papers for more details.

\paragraph{Set Abstraction (SA)} 
Set abstraction is the downsampling layer introduced in \cite{Qi2017NIPS}. 
It proceeds by (1) \textit{sampling} a subset of ``centroid'' points from the point cloud at the current resolution, (2) \textit{grouping} the points around these centroids into local neighborhoods, (3) translating points into the local frame of their centroid and processing all points with a shared MLP, and (4) pooling over each local neighborhood to get a downsampled point cloud with associated features.
\textit{Sampling} uses iterative farthest point sampling (FPS) \cite{Qi2017NIPS}, and
% : at each iteration $k$, a point $p_k$ is added to the sampled subset such that $p_k$ is the farthest (in the Euclidean sense) from all previously sampled points $\{p_1, p_2, ..., p_{k-1}\}$.
\textit{grouping} commonly uses a ball query, which groups together all points within a specified radius from a centroid.
% Lastly, pooling can be max-pooling, mean-pooling, or an attention pooling~\cite{Hu2020CVPR}.

\paragraph{Feature Propagation (FP)} 
Feature propagation is the upsampling layer introduced in \cite{Qi2017NIPS}.
Its goal is to propagate features from a low-resolution point cloud $\{q_1, ..., q_L\}$ with $L$ points to a higher-resolution point cloud $\{p_1, ..., p_H\}$ with $H$ points where $L{<}H$.
This is achieved with \textit{feature interpolation}: given the low-res point features $\{g_1, ..., g_L\}$, the high-res point features  $F{=}\{f_1, ..., f_H\}$ are determined by a distance-weighted feature interpolation of the $k$ nearest low-res neighbors for each high-res point (based on the spatial coordinates of the points). 
% To get the final upsampled point features, the high-res interpolated features $F$ are concatenated with skip-linked features from a corresponding SA layer and processed by a shared MLP.


% \paragraph{Graph Convolution}
% DGCNN~\cite{Wang2019SIGGRAPHb} leverages convolution operations on a dynamically constructed graph to process points.
% At each layer, the graph is constructed by adding edges between each point and its $k$ nearest neighbors in the learned feature space. 
% The convolution centered at a point uses a learned edge function for each edge followed by aggregation. Constructing a dynamic graph in feature space is computationally prohibitive on larger scenes, so we opt to construct the graph based on 3D point distances (\cref{sec:curvecloudnet}). 

\vspace{-2mm}
\subsubsection{Curve Operations}
\vspace{-1mm}
We introduce new operations for \textit{sampling}, \textit{grouping}, \textit{feature interpolation}, and \textit{convolutions} along curves to expressively and efficiently learn on curve clouds.

\paragraph{1D Farthest Point Sampling}
FPS is frequently a bottleneck in point cloud architectures and can be costly for large point clouds~\cite{Hu2020CVPR} due to pair-wise distance computations. 
% Subsampling $L$ points from a point cloud of $N$ points has a time complexity of $O(N^2)$ due to paired distance computations, and requires $O(L)$ sequential steps.
For curves, we alleviate this cost with an approximation of FPS \textit{along each curve} independently in a 1D manner.
This amounts to sampling a subset of points on each curve that are evenly-spaced along the length of that curve (\ie, geodesically).
For a curve $c_j$ with $N_j$ points, we subsample a point set $\{q_1, ..., q_{L_j}\}$ with $L_j{<}N_j$ such that all pairs of contiguous points are about $\epsilon$ apart, where $\epsilon$ is a fixed target spacing shared across \textit{all} curves. 
In other words, $d(q_i, q_{i-1}){\approx}\epsilon$ for $i=2,\dots,L_j$ where $d$ measures the geodesic distance between two points along the same curve.
Notably, this algorithm has only $O(N)$ complexity and can be parallelized across each curve independently.
%Additional details regarding our 1D Farthest Point Sampling are provided in the supplementary material. 

% \subsubsection{1D Farthest Point Sampling} \label{subsec:1d-fps}
% Most point-cloud backbones use iterative farthest point sampling (FPS) to obtain a subset of points with good coverage over the occupied space. Iterative FPS begins with a random sampled point, $p_1$, and then iteratively samples $p_i$ as the farthest point from all previously sampled points $p_1, ..., p_{k-1}$. Importantly, to subsample $N'$ points, FPS performs $O(N')$ sequential steps and has a computational complexity $O(N^2)$. This can result in a significant computational burden for large point clouds \cite{randla_net}.

% To reduce computational cost, we apply a 1D FPS \textit{along} each curve independently. 
% In the 1D case, FPS reduces to evenly-spaced geodesic sampling along each curve. In contrast to 3D FPS, our 1D FPS only performs $log(N_j^{max})$ iterations and has $O(N)$ complexity, where $N_j^{max} = \max(N_j), j \in [1, ..., M])$, i.e. the maximum number of points belonging to a single curve. For more details on our 1D FPS algorithm, please refer to the Supplementary material. 

\paragraph{Grouping Along Curves}
After sampling, we must group points into local neighborhoods around the subsampled points on each curve.
To do this, we adapt the previously discussed ball query to operate along each curve.
For a query point $p_i$ belonging to curve $c_j$ (one of the ``centroids'' from sampling), we define the local neighborhood of $p_i$ as $\mathcal{N}_i = \{p_k \in c_j \,|\, d(p_i, p_k) < r\}$ where $r$ is a fixed neighborhood radius.
In addition to being computationally faster than a standard 3D ball query grouping, using 1D curve groupings ensures that all neighborhoods lie on a continuous section of scanned surfaces.

% \subsubsection{Curve Grouping}\label{subsec:1d-grouping}
% We adapt the core grouping operation of PointNet++ \cite{pointnet2} to the 1D polyline. Specifically, we obtain a set of downsampled query points, $\{q_1, ..., q_K\}$, s.t. $K < N$. Then, for each query point $q_k$ that lies on curve $c_j$, we group all points along $c_j$ that lie within the 1D geodesic neighborhood of $q_k$. We define neighborhood as being closer than a fixed geodesic radius $r$. For each query $q_k$, this yields a set of neighboring points $N_k = \{n_1, ..., n_{|N|}\}$. 

% Finally, we center $N_k$ around $q_k$ and extract a neighborhood feature via a PointNet MLP \cite{pointnet} and attention-pooling aggregation \cite{randla}. In addition to being computationally faster than a standard PointNet++ grouping, our 1D groupings ensures that all neighborhoods lie on a continuous section of scanned surfaces.  


\paragraph{Curve Feature Interpolation}
To upsample on curves, we must interpolate features from a lower-resolution polyline to a higher-resolution one.
Let $p_h$ be the h$^{th}$ point on the high-res curve, which falls between subsampled low-res points $q_i$ and $q_{i-1}$ with associated features $g_i$ and $g_{i-1}$.
The interpolated high-res feature $f_h$ is simply the distance-weighted interpolation of the two low-res points.
% : $f_h = (1 - \alpha) \cdot g_i + \alpha \cdot g_{i-1}$ where $\alpha = d(p_h, g_i) / d(g_i, g_{i-1})$ and $d$ measures distances with respect to the \emph{high-res} curve.
\input{content/main/figures/object_samples.tex}

\input{content/main/tables/summer-robotics.tex}

\paragraph{Symmetric Curve Convolution}
To process points along curves, we take advantage of expressive convolutions. 
However, it is computationally burdensome to compute neighborhoods on the fly and run convolutions on unordered data \cite{Liu2021TPAMI}.
% and operate on dynamic nearest neighbor structures rather than the simple 1D structure of curves.
%overkill given the simple 1D structure of the curves.
% directly on each polyline would be very limited due to each point having only two edges. or expensive to dynamically compute more edges?
Instead, we treat each curve as a discrete grid of features that can be convolved similar to a 1D sequence. 
To account for the bi-directionality of curves,  we employ a symmetric convolution and thus produce equivalent results when applied ``forward'' or ``backward'' along the curve. 
% This ensures the scanning direction of the laser in the scene has no effect on the convolution result.

In particular, for a curve $c_j = [p_1, p_2, ..., p_{N_j}]$ with associated point features $F_j = [f_1, f_2, ..., f_{N_j}]$, we start by extracting additional features using the the L1 norm of feature gradients along the curve~\cite{Wiersma2022SIGGRAPH}, denoted as $\nabla F_j = \big[ |\nabla f_1|, |\nabla f_2|, ..., |\nabla f_{N_j}| \big ]$. 
Note the norm is necessary to remove directional information.
Concatenating these features together as $[F_j, \nabla F_j] \in \mathbb{R}^{N\times D}$ gives a grid on which to perform 1D convolutions.
To respect bi-directionality, symmetric kernels are used for the convolution: for a kernel $W \in \mathbb{R}^{S \times D}$ with size $S$ and $D$ channels, we ensure $W_i = W_{S-i+1}$ for $i = 1, \dots, S$ where $W_i \in \mathbb{R}^D$.

 % $W_{\text{sym}}*F_{c_j}$

% \input{content/main/figures/object_samples.tex}

% \input{content/main/tables/summer-robotics.tex}
\vspace{-2mm}
\subsubsection{Curve Layers} \label{subsec:curve-layers}
\vspace{-1mm}
We integrate curve operations into curve layers that act as building blocks for the backbone detailed in \cref{sec:curvecloudnet}.

\paragraph{Curve Set Abstraction (Curve SA)}
Curve set abstraction is a curve-centric downsampling procedure. For each curve, Curve SA (1) samples a subset of centroid points using \textit{1D farthest point sampling}, (2) groups points along the curve using \textit{curve grouping}, (3) translates points into the local frame of their centroid and processes them with a shared MLP, and (4) pools over each local neighborhood to get downsampled point features.

\paragraph{Curve Feature Propagation (Curve FP)}
Curve feature propagation is a curve-centric upsampling layer. For a curve $c_j$, its goal is to propagate features from a low-res polyline $[q_1, ..., q_{L_j}]$ with $L_j$ points to a higher-res polyline $[p_1, ..., p_{H_j}]$ with $H_j$ points where $L_j < H_j$. This is achieved using \textit{curve feature interpolation} described above. Afterwards, the high-res interpolated features are concatenated with skip-linked features from a corresponding curve set abstraction layer and processed by a shared MLP.

\paragraph{Curve Convolution}
The curve convolution layer allows for efficient communication and feature extraction along a curve. This module consists of three sequential \textit{symmetric curve convolutions}, each followed by batch normalization~\cite{Ioffe2015bn} and a leaky ReLU activation.


\subsection{Curve Cloud Backbone: \arch} \label{sec:curvecloudnet}
We propose a novel architecture, \arch, that processes curve clouds for several perception tasks. % As illustrated in \cref{fig:curvecloudnet-architecture}, \arch uses a mix of curve layers described and point-based layers.
%\paragraph{\arch Architecture}
In \cref{fig:curvecloudnet-architecture}, we illustrate CurveCloudNet as designed for segmentation tasks where the output is a single semantic class (one-hot vector) for each point in the input point cloud.
Hence, it follows the U-Net~\cite{Ronneberger2015MICCAI} structure, consisting of a series of downsampling layers followed by upsampling with skip connections.
Although in our experiments (\cref{sec:experiments}) we focus on segmentation, \arch can be adapted to other point cloud perception tasks (see supplement for a classification example).

Our architecture is a mix of curve and point-based layers.
At higher resolutions, curve modules are employed since they are efficient and can capture geometric details when curve sampling is most dense across surfaces in the scene. 
At lower resolutions, point modules are used to propagate information across curves when 1D structure is less apparent. For point operations, we adopt the \textit{set abstraction} and \textit{feature propagation} operations from \cite{Qi2017NIPS} as well as the graph convolution from \cite{Wang2019SIGGRAPHb}, and we further improve these point operations following the reportings of recent works \cite{Hu2020CVPR, Ma2022ICLR, Qian2022PointNeXtRP} (see Supplementary for further details).
By combining curve and point operations, \arch is an expressive network that maintains the benefits of point cloud backbones while injecting structure and efficiency previously only possible with voxel-based approaches.

% \paragraph{Training}
% We train CurveCloudNet on segmentation tasks with a standard cross-entropy loss. Following previous works, we also supplement the loss with a Lovasz loss \cite{Berman2018CVPR, Zhou2020ARXIV} for nuScenes and Audi Autonomous Driving datasets. At training, we apply random scaling and translation augmentations, as well as random flips on nuScenes and Audi.



==> preamble.tex <==
\ProvidesPackage{shortcuts}

\usepackage{booktabs}
\usepackage{listings} 
% \usepackage[dvipsnames]{xcolor}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\definecolor{Gray}{gray}{0.85}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\renewcommand{\eg}{\textit{e.g.}\xspace}
\renewcommand{\ie}{\textit{i.e.}\xspace}
\renewcommand{\paragraph}[1]{{\vspace{1mm}\noindent \bf #1}.}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{subcaption}
%\usepackage{minted}

\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}



% shortcuts for bold characters (vectors, matrices)
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}} %\bf already taken
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

% shortcuts for bold greek characters (vectors, matrices)
\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} % \beta already taken
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

% shortcuts for blackboard bold characters (eg, number sets)
\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

% shortcuts for calligraphic characters (sets, index sets, ...)
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% references to figures, sections, algorithms, equations, tables
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}

% argmin / argmax operators
\usepackage{amsfonts}
\DeclareMathOperator*{\argmax}{argmax~}
\DeclareMathOperator*{\argmin}{argmin~}
\DeclareMathOperator{\EX}{\mathbb{E}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\relu}{relu}

% mathcal / mathbf shortcuts
\def\mc{\mathcal}
\def\mb{\mathbf}

% two-dot ellipse
\newcommand{\twodots}{\mathinner {\ldotp \ldotp}}

% nice transpose operator
\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

% statistical dependency symbol (_||_)
\newcommand{\Perp}{\perp\!\!\! \perp}

% shortcuts for: \eg, \ie, \cf, \etc, \vs, \wrt, \dof, \etal, \iid
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot}
\def\iid{i.i.d\onedot}
\makeatother

% nice url font and color
\renewcommand\UrlFont{\color{blue}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}

% boldparagraph for unnumbered sections
\newcommand{\boldparagraph}[1]{\vspace{0.2cm}\noindent{\bf #1:} }

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}

% custom color definitions
\usepackage{xcolor}
\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{orange}{RGB}{255,127,0}
\definecolor{ourpurple}{RGB}{127,127,204}
\definecolor{palgreen}{RGB}{51,179,179}
\definecolor{magenta}{RGB}{199,21,133}

\definecolor{darkred}{RGB}{220,50,32}
\definecolor{darkblue}{RGB}{0,90,181}
\newcommand{\darkred}[1]{\noindent{\color{darkred}{#1}}}
\newcommand{\darkblue}[1]{\noindent{\color{darkblue}{#1}}}

% commands for comments
\newcommand{\green}[1]{\noindent{\color{green}{#1}}}
\newcommand{\desp}[1]{ \noindent {\color{cyan} {\bf Despoina:} {#1}} }

\newcommand{\todo}[1]{{\textcolor{red}{\textbf{#1}}}}
\newcommand{\colton}[1]{{\textcolor{red}{\textbf{Colton}: #1}}}
\newcommand{\davis}[1]{{\textcolor{blue}{\textbf{Davis}: #1}}}
\newcommand{\leo}[1]{{\textcolor{magenta}{\textbf{Leo}: #1}}}
\newcommand{\jj}[1]{{\textcolor{green}{\textbf{JJ}: #1}}}

\newcommand{\lidar}{LiDAR\xspace}
\newcommand{\kortx}{Kortx\xspace}
\newcommand{\arch}{CurveCloudNet\xspace}

\newcommand{\rotbox}[2]{\rotatebox[origin=l]{#1}{#2}}

==> shortcuts.tex <==
\ProvidesPackage{shortcuts}

% shortcuts for bold characters (vectors, matrices)
\newcommand{\ba}{\mathbf{a}}\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}\newcommand{\bE}{\mathbf{E}}
\newcommand{\bff}{\mathbf{f}}\newcommand{\bF}{\mathbf{F}} %\bf already taken
\newcommand{\bg}{\mathbf{g}}\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}\newcommand{\bL}{\mathbf{L}}
\newcommand{\bm}{\mathbf{m}}\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}\newcommand{\bZ}{\mathbf{Z}}

% shortcuts for bold greek characters (vectors, matrices)
\newcommand{\balpha}{\boldsymbol{\alpha}}\newcommand{\bAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}\newcommand{\bBeta}{\boldsymbol{\Beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}\newcommand{\bEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}\newcommand{\bZeta}{\boldsymbol{\Zeta}}
\newcommand{\beeta}{\boldsymbol{\eta}}\newcommand{\bEta}{\boldsymbol{\Eta}} % \beta already taken
\newcommand{\btheta}{\boldsymbol{\theta}}\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\biota}{\boldsymbol{\iota}}\newcommand{\bIota}{\boldsymbol{\Iota}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}\newcommand{\bKappa}{\boldsymbol{\Kappa}}
\newcommand{\blambda}{\boldsymbol{\lambda}}\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}\newcommand{\bMu}{\boldsymbol{\Mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}\newcommand{\bNu}{\boldsymbol{\Nu}}
\newcommand{\bxi}{\boldsymbol{\xi}}\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bomikron}{\boldsymbol{\omikron}}\newcommand{\bOmikron}{\boldsymbol{\Omikron}}
\newcommand{\bpi}{\boldsymbol{\pi}}\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\brho}{\boldsymbol{\rho}}\newcommand{\bRho}{\boldsymbol{\Rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}\newcommand{\bTau}{\boldsymbol{\Tau}}
\newcommand{\bypsilon}{\boldsymbol{\ypsilon}}\newcommand{\bYpsilon}{\boldsymbol{\Ypsilon}}
\newcommand{\bphi}{\boldsymbol{\phi}}\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bchi}{\boldsymbol{\chi}}\newcommand{\bChi}{\boldsymbol{\Chi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bomega}{\boldsymbol{\omega}}\newcommand{\bOmega}{\boldsymbol{\Omega}}

% shortcuts for blackboard bold characters (eg, number sets)
\newcommand{\nA}{\mathbb{A}}
\newcommand{\nB}{\mathbb{B}}
\newcommand{\nC}{\mathbb{C}}
\newcommand{\nD}{\mathbb{D}}
\newcommand{\nE}{\mathbb{E}}
\newcommand{\nF}{\mathbb{F}}
\newcommand{\nG}{\mathbb{G}}
\newcommand{\nH}{\mathbb{H}}
\newcommand{\nI}{\mathbb{I}}
\newcommand{\nJ}{\mathbb{J}}
\newcommand{\nK}{\mathbb{K}}
\newcommand{\nL}{\mathbb{L}}
\newcommand{\nM}{\mathbb{M}}
\newcommand{\nN}{\mathbb{N}}
\newcommand{\nO}{\mathbb{O}}
\newcommand{\nP}{\mathbb{P}}
\newcommand{\nQ}{\mathbb{Q}}
\newcommand{\nR}{\mathbb{R}}
\newcommand{\nS}{\mathbb{S}}
\newcommand{\nT}{\mathbb{T}}
\newcommand{\nU}{\mathbb{U}}
\newcommand{\nV}{\mathbb{V}}
\newcommand{\nW}{\mathbb{W}}
\newcommand{\nX}{\mathbb{X}}
\newcommand{\nY}{\mathbb{Y}}
\newcommand{\nZ}{\mathbb{Z}}

% shortcuts for calligraphic characters (sets, index sets, ...)
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\co}{\mathcal{o}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% references to figures, sections, algorithms, equations, tables
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\eqnref}[1]{Eq.~\eqref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}

% argmin / argmax operators
\usepackage{amsfonts}
\DeclareMathOperator*{\argmax}{argmax~}
\DeclareMathOperator*{\argmin}{argmin~}
\DeclareMathOperator{\EX}{\mathbb{E}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\relu}{relu}

% mathcal / mathbf shortcuts
\def\mc{\mathcal}
\def\mb{\mathbf}

% two-dot ellipse
\newcommand{\twodots}{\mathinner {\ldotp \ldotp}}

% nice transpose operator
\newcommand{\T}{^{\raisemath{-1pt}{\mathsf{T}}}}

% statistical dependency symbol (_||_)
\newcommand{\Perp}{\perp\!\!\! \perp}

% shortcuts for: \eg, \ie, \cf, \etc, \vs, \wrt, \dof, \etal, \iid
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{wrt\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et~al\onedot}
\def\iid{i.i.d\onedot}
\makeatother

% nice url font and color
\renewcommand\UrlFont{\color{blue}\rmfamily}

% rotation
\newcommand*\rot{\rotatebox{90}}

% boldparagraph for unnumbered sections
\newcommand{\boldparagraph}[1]{\vspace{0.2cm}\noindent{\bf #1:} }

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}

% custom color definitions
\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{orange}{RGB}{255,127,0}
\definecolor{ourpurple}{RGB}{127,127,204}
\definecolor{palgreen}{RGB}{51,179,179}
\definecolor{magenta}{RGB}{199,21,133}

\definecolor{darkred}{RGB}{220,50,32}
\definecolor{darkblue}{RGB}{0,90,181}
\newcommand{\darkred}[1]{\noindent{\color{darkred}{#1}}}
\newcommand{\darkblue}[1]{\noindent{\color{darkblue}{#1}}}

% commands for comments
\newcommand{\green}[1]{\noindent{\color{green}{#1}}}
\newcommand{\desp}[1]{ \noindent {\color{cyan} {\bf Despoina:} {#1}} }

